tomoCAM: Fast Model-based Iterative Reconstruction via GPU Acceleration and Non-Uniform Fast Fourier Transforms

X-Ray based computed tomography (CT) is a well-established technique for determining the three-dimensional structure of an object from its two-dimensional projections. In the past few decades, there have been significant advancements in the brightness and detector technology of tomography instruments at synchrotron sources. These advancements have led to the emergence of new observations and discoveries, with improved capabilities such as faster frame rates, larger fields of view, higher resolution, and higher dimensionality. These advancements have enabled the material science community to expand the scope of tomographic measurements towards increasingly in-situ and in-operando measurements. In these new experiments, samples can be rapidly evolving, have complex geometries, and restrictions on the field of view, limiting the number of projections that can be collected. In such cases, standard filtered back-projections (FBP) for the reconstructions often result in poor-quality reconstructions. Iterative reconstruction algorithms, such as model-based iterative reconstructions (MBIR), have demonstrated considerable success in producing high-quality reconstructions under such restrictions, but typically require high-performance computing resources with hundreds of compute nodes to solve the problem in a reasonable time.

==> mbir_algorithm.tex <==
\begin{algorithm}%
\centering
\begin{minipage}{\linewidth}
\begin{center}
       \textit{GPU-accelerated Model Based Iterative Reconstruction Algorithm}
\end{center}
\end{minipage}
\begin{minipage}{\linewidth}
\DontPrintSemicolon
\SetKwProg{kwInit}{Initialize}{}{}
\kwInit{}{
\tcc{F: reconstructed volume}
\tcc{D: gradient}
\tcc{Y: projection data} 
 F  $\longleftarrow 1, D \longleftarrow \emptyset $ \\
 F  $\gets \bigcup_{i}^{N_{gpus}} f_i$,~
 D  $\gets \bigcup_{i}^{N_{gpus}} d_i$,~
 Y  $\gets \bigcup_{i}^{N_{gpus}} y_i $ \;
}

\While{$ e > $ tolerance $\mathbf{or}$ iter $\le$ max\_iters }{
    \SetKwProg{kwGrad}{Gradient}{}{}
	\kwGrad{}{
	\For{$i \gets 1$ \textbf{to} $N_{gpus}$ \tcc{OpenMP  parallel}}{
  		\texttt{cudaSetDevice}($i$) \;
  		$f_i \gets \bigcup_j^n f_{ij}$,~
  		$y_i \gets \bigcup_j^n y_{ij}$ \;
  		\For{$j \gets 1$ \textbf{to} $n$ \tcc{OpenMP parallel}}{
  			\texttt{cuMemcpyAsync}($f_{ij}$, \ldots, \texttt{HostToDevice}) \;
			\texttt{cuMemcpyAsync}($y_{ij}$, \ldots, \texttt{HostToDevice}) \;
    		$d_{ij} \gets R* [R(f_{ij} -y$)] \;
    		\texttt{cudaMemcpyAsync}($d_{ij}$, \ldots, \texttt{DeviceToHost})
  			}
		}
	}
    \SetKwProg{kwTV}{TV Constraint}{}{}
	\kwTV{}{
	\For{$i \gets 1$ \textbf{to} $N_{gpus}$ \tcc{OpenMP  parallel}}{
	    \texttt{cudaSetDevice}($i$) \;
  		$f_i \gets \bigcup_j^n f_{ij}$,~
  		$d_i \gets \bigcup_j^n d_{ij}$ \;
  		\For{$j \gets 1$ \textbf{to} $n_i$ \tcc{OpenMP  parallel}} { 
  			\texttt{cuMemcpyAsync}($f_{ij}$, \ldots, \texttt{HostToDevice}) \;
			\texttt{cuMemcpyAsync}($d_{ij}$, \ldots, \texttt{HostToDevice}) \;
    		 $d_{ij} \gets d_{ij}$ + TV($f_{ij})$ \;
    		\texttt{cudaMemcpyAsync}($d_{ij}$, \ldots, \texttt{DeviceToHost}) \;
  			}
		}
	}
	\tcc{Minimization step}
	F $\gets$ F - $\lambda$ D \;
    e $\gets$ [R(f) - y]$^T$ [R(f) - y]
}
\end{minipage}
   \label{algo:mbir}
\end{algorithm}

